LiDAR R-CNN: An Efficient and Universal 3D Object Detector

LiDAR-based 3D detection in point cloud is essential in the perception system of autonomous driving. In this paper, we present LiDAR R-CNN, a second stage detector that can generally improve any existing 3D detector. To fulfill the real-time and high precision requirement in practice, we resort to point-based approach other than the popular voxel-based approach. However, we find an overlooked issue in previous work: Naively applying point-based methods like PointNet could make the learned features ignore the size of proposals. To this end, we analyze this problem in detail and propose several methods to remedy it, which bring significant performance improvement. Comprehensive experimental results on real-world datasets like Waymo Open Dataset (WOD) and KITTI dataset with various popular detectors demonstrate the universality and superiority of our LiDAR R-CNN. In particular, based on one variant of PointPillars, our method could achieve new state-of-the-art results with minor cost. Codes will be released at https://github.com/tusimple/LiDAR_RCNN .

==> src/experiments__Zhichao_Li_s_conflicted_copy_2020-11-17_.tex <==
\section{Experiments}

\begin{table*}
	\small
	\vspace{-1mm}
	\begin{center}
		\scalebox{0.79}[0.79]{
			\setlength\tabcolsep{2pt}
			\begin{tabular}{c|c||cccc|cccc|cccc|cccc}
				\hline
				\multirow{2}{*}{Difficulty} & \multirow{2}{*}{Method} &
				\multicolumn{4}{c|}{3D mAP (IoU=0.7)} & \multicolumn{4}{c|}{3D mAPH (IoU=0.7)} &
				\multicolumn{4}{c|}{BEV mAP (IoU=0.7)} &
				\multicolumn{4}{c}{BEV mAPH (IoU=0.7)} \\
				& & Overall & 0-30m & 30-50m & 50m-Inf &
				Overall & 0-30m & 30-50m & 50m-Inf  &
				Overall & 0-30m & 30-50m & 50m-Inf &
				Overall & 0-30m & 30-50m & 50m-Inf \\
				\hline
				LEVEL\_1
				& PointPillar~\cite{pointpillars}  & 56.6 & 81.0 & 51.8 & 27.9 & - & - & - & - & 75.6 & 92.1 & 74.1 & 55.5 & - & - & - & -  \\
				& MVF~\cite{mvf}  & 62.9 & 86.3 & 60.0 & 36.0 & - & - & - & - & 80.4 & 93.6 & 79.2 & 63.1 & - & - & - & -\\
				& PV-RCNN~\cite{pv-rcnn} & 70.3 & 91.9 & 69.2 & 42.2 & 69.7 & 91.3 & 68.5 & 41.3 & 83.0 & \textbf{97.4} & 83.0 & 65.0 & 82.1 & \textbf{96.7} & 82.0 & 63.2 \\
				\cline{2-18}
                & RCD first stage ~\cite{rcd} & 53.4 & 73.0 & 49.0 & 28.1 & 52.8 & 72.3 & 48.4 & 27.8 & 70.5 & 86.2 & 68.5 & 51.9 & 69.5 & 85.2 & 67.6 & 51.0 \\
                & \Name(rv) & 68.7 & 84.8 & 67.6 & 47.3 & - & - & - & - & - & - & - & - & - & - & - & - \\
                \cline{2-18}
				& PointPillar* & 72.1 & 88.3 & 69.9 & 48.0 & 71.5 & 87.8 & 69.3 & 47.3 & 87.9 & 96.6 & 87.1 & 78.1 & 87.1 & 96.0 & 86.2 & 76.5 \\
				& \Name(pp) & 75.6 & \textbf{92.1} & \textbf{74.3} & 53.3 & 75.1 & \textbf{91.6} & \textbf{73.8} & 52.6 & 88.2 & 97.1 & 87.6 & 78.3 & 87.5 & 96.6 & 86.9 & 76.8 \\
				& \Name(2x) & \textbf{75.6} & 91.9 & 74.2 & \textbf{53.5} & \textbf{75.1} & 91.5 & 73.6 & \textbf{52.7} & \textbf{90.0} & 97.0 & \textbf{89.4} & \textbf{78.5} & \textbf{89.2} & 96.6 & \textbf{88.6} & \textbf{77.0} \\
				\hline
				LEVEL\_2 & PV-RCNN~\cite{pv-rcnn} & 65.4 & \textbf{91.6} & 65.1 & 36.5 & 64.8 & \textbf{91.0} & 64.5 & 35.7 & 77.5 & \textbf{94.6} & 80.4 & 55.4 &76.6 & \textbf{94.0} & 79.4 & 53.8\\
				\cline{2-18}
                & RCD first stage ~\cite{rcd} & 46.0 & 70.6 & 44.1 & 21.0 & 45.5 & 69.8 & 43.6 & 20.7 & 63.5 & 85.5 & 62.7 & 41.1 & 62.7 & 84.5 & 61.9 & 40.3 \\
				& \Name(rv) & 60.1 & 84.1 & 61.8 & 35.7 & - & - & - & - & - & - & - & - & - & - & - & - \\
				\cline{2-18}
                & PointPillar* & 63.6 & 87.4 & 62.9 & 37.2 & 63.1 & 86.9 & 62.3 & 36.7 & 81.3 & 94.0 & 81.7 & 65.5 & 80.4 & 93.5 & 80.8 & 64.1 \\
				& \Name(pp) & 66.5 & 89.1 & \textbf{68.3} & 40.8 & 66.1 & 88.7 & \textbf{67.7} & 40.3 & 81.2 & 94.2 & 81.7 & 63.6 & 80.5 & 93.7 & 81.0 & 62.3 \\
				& \Name(2x) & \textbf{68.0} & 91.1 & 68.1 & \textbf{41.1} & \textbf{67.6} & 90.7 & 67.6 & \textbf{40.5} & \textbf{81.6} & 94.3 & \textbf{82.2} & \textbf{65.6} & \textbf{80.9} & 93.9 & \textbf{81.4} & \textbf{64.2} \\
				\hline
			\end{tabular}
		}
	\end{center}
	\vspace{-0.3cm}
	\caption{Vehicle detection results on Waymo Open Dataset validation sequences. Here PointPillar~\cite{pointpillars} is reproduced by ~\cite{mvf} and PointPillar* is implemented in mmdetection3d. Our \Name(pp) results are based on PointPillar*'s proposals. Range view method is reproduced by ourselves followed ~\cite{rcd}.}
	\label{tab:waymo-vehicle}
\end{table*}


\begin{table*}
	\begin{center}
		\scalebox{0.9}[0.9]{
			\setlength\tabcolsep{2pt}
			\begin{tabular}{c|c||cc|cc|cc}
				\hline
				\multirow{2}{*}{Difficulty} & \multirow{2}{*}{Method} &
				\multicolumn{2}{c|}{vehicle (IoU=0.7)} & \multicolumn{2}{c|}{pedestrian (IoU=0.5)} &
				\multicolumn{2}{c}{cyclist (IoU=0.5)} \\
				& & 3D mAP  & 3D mAPH &
				3D mAP & 3D mAPH  &
				3D mAP & 3D mAPH \\
				\hline
				LEVEL\_1
				& SECOND~\cite{second} & 58.5 & 57.9 & 63.9 & 54.9 & 48.6 & 47.6  \\
				& \Name(sec) & 62.6 & 62.1 & 68.2 & 59.5 & 52.8 & 51.6 \\
				\cline{2-8}
				& PointPillar~\cite{pointpillars} & 71.6 & 71.0 & 70.6 & 56.7 & 64.4 & 62.3  \\
				& \Name(pp) & 73.4 & 72.9 & 70.6 & 57.8 & 66.8 & 64.8  \\
				& \Name(2x) & 73.5 & 73.0 & 71.2 & 58.7 & 68.6 & 66.9  \\
				\hline
				LEVEL\_2
				& SECOND~\cite{second} & 51.6 & 51.1 & 56.0 & 48.0 & 46.8 & 45.8  \\
				& \Name(sec) & 54.5 & 54.0 & 59.3 & 51.7 & 50.9 & 49.7 \\
				\cline{2-8}
				& PointPillar~\cite{pointpillars} & 63.1 & 62.5 & 62.9 & 50.2 & 61.9 & 59.9   \\
				& \Name(pp) & 64.6 & 64.1 & 62.5 & 50.9 & 64.3 & 62.4  \\
				& \Name(2x) & 64.7 & 64.2 & 63.1 & 51.7 & 66.1 & 64.4  \\
				\hline
			\end{tabular}
		}
	\end{center}
	\vspace{-0.3cm}
	\caption{Multi-class 3D detection results on Waymo Open Dataset validation sequences. Both PointPillar and SECOND baselines are implemented in mmdetection3d. 2x means we double the channels in points encoding network.}
	\label{tab:waymo-3d}
	\vspace{-0.3 cm}
\end{table*}


% To be refine
\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\begin{tabular}{l|c|c}
		\toprule
		Methods    & 3D mAP@70 & BEV mAP@70  \\ \midrule
		RV first stage~\cite{rcd} & 53.4 & 70.5 \\
		RV second stage~\cite{rcd} & 64.1 & 76.7  \\
		RV+\Name(rv) & \textbf{68.7} &  \textbf{81.1}   \\
		% \midrule
		% PP & - & -  \\
		\bottomrule
	\end{tabular}
	\vspace{2pt}
	\caption{Comparison between voxel-based second-stage and proposed \Name on RCD framework~\cite{rcd}. RV+ours replaces the second-stage with our method.}
	\label{tab:ablation-voxel}
\end{table}

\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\begin{tabular}{l|c|c}
		\toprule
		Methods    & 3D mAP@70 & BEV mAP@70  \\ \midrule
		PointPillar & 71.6 & -  \\
		PointNet refinement & 74.1 & 87.9  \\
		voxel    & 72.9 & 87.2   \\
		anchor    & 75.2 & 88.2   \\
		size normalization    & 75.4 &  88.1   \\
		\midrule
		virtual point   & 75.4 &  88.1   \\
		boundary offset      & 75.6 &  88.3   \\
		\bottomrule
	\end{tabular}
	\vspace{2pt}
	\caption{Ablation studies for different scale-awared methods proposed in \secref{subsec:Problem} on Waymo Open Dataset vehicle detection. The baseline use a basic PointNet with [x,y,z] inputs as second-stage on Pointpillars.}
	\label{tab:ablation-single}
\end{table}


\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\begin{tabular}{l|c|c|c}
		\toprule
		Methods    & vehicle & pedestrian  & cyclist \\ \midrule
		PointPillar  & 71.6 & 70.6 & 64.4 \\
		PointNet refinement   & 72.1 & 69.2 & 62.2 \\
		voxel   & - & - & - \\
		anchor   & 72.5 & 70.2 & 63.5 \\
		size normalization    & 72.7 & 69.9 & 64.4   \\
		\midrule
		virtual point   & 73.3 &  70.4 & 66.2  \\
		boundary offset      & 73.4 &  70.6 & 66.8  \\
		\bottomrule
	\end{tabular}
	\vspace{2pt}
	\caption{3D mAP results on WOD when three classes are trained in one model.}
	\label{tab:ablation-three}
\end{table}

\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\begin{tabular}{l|c|c|c}
		\toprule
		Methods    & vehicle & pedestrian  & cyclist \\ \midrule
		SECOND   & 58.5 & 63.9 & 48.6 \\
		\Name(sec)    & 62.6 & 68.2 & 52.8   \\
		\midrule
		\Name(pp)   & 62.1 &  67.2 & 52.9  \\
		\bottomrule
	\end{tabular}
	\vspace{2pt}
	\caption{We show generalization of our \Name in this Table. \Name(sec) use the outputs from SECOND for training and testing. \Name(pp) trains with Pointpillars' outputs while inferencing on SECOND without finetuning.}
	\label{tab:ablation-generalization}
\end{table}

\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\begin{tabular}{l|c|c|c}
		\toprule
		Methods    & 3D mAP & time  & Params \\ \midrule
		voxel   & 72.9 & 19ms & 3.5M \\
		ours  & 75.6 & 4.5ms & 0.5M   \\
		\bottomrule
	\end{tabular}
	\vspace{2pt}
	\caption{Inference time comparison between voxel-based and our proposed method. The inference time is evaluated with 128 proposals(batchsize=128).}
	\label{tab:ablation-speed}
\end{table}


\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{img/number_points.pdf}
	\caption{Adaptive inference time with different sampled points. Evaluate the \Name sampling 64 to 1024 points per object on Waymo Open Dataset Validation set.}
	\label{fig:number_points}
\end{figure}

In this section, we first briefly introduce the datasets we use in \secref{subsec:datasets}, then the implementation details of our \Name is provided in \secref{subsec:Implementation Details}. \secref{subsec:Waymo Open Dataset} shows that \Name can generally improve the performance of all baseline models, and surpasses the previous state-of-the-art methods. In \secref{subsec:Ablation}, we conduct extensive ablation studies to show that the proposed methods can effectively solve the problem described in \secref{subsec:Problem}.

\subsection{Waymo Open Dataset(WOD)~\cite{wod}}\label{subsec:datasets}
Waymo Open Dataset is a recent released public dataset for autonomous driving research. It contains RGB images from five high-resolution pinhole cameras and 3D point clouds from five LiDAR sensors. The data is collected with variety of weather conditions in several different cities. The whole dataset consists of 1000 scenes(20s fragment) for training and validation and 150 scenes for testing. For the 3D detection task, the dataset has 12M labeled 3D LiDAR objects which are annotated in full 360-degree field, including 4.81M vehicles and 2.22M pedestrians for training and 1.25M vehicles and 539K pedestrians for validation. It is one of the largest and most diverse autonomous driving datasets.
For evaluation, Average precision (AP) and APH are used as the metric. Specifically, ~\cite{wod} propose APH to incorporate heading information into detection metrics. The IoU threshold for vehicle detection is 0.7 while 0.5 for pedestrian and cyclist.

% \paragraph{nuScenes~\cite{nuscenes}.}
% The nuScenes dataset has full autonomous driving sensor which contains 360-degree field of data from 6 cameras, 5 radars, and 1 LiDAR. Same as WOD, each scene spans 20 seconds. One thousand scenes are annotated with 3D bounding boxes for 23 classes with object's velocity. The points cloud data in nuScenes are collected with a 32 rays LiDAR, which is far more sparse with WOD. We use this dataset to demonstrate the robustness of our method to different hardware configurations. Different from common evaluation metrics used in KITTI or WOD, Average Precision (AP) in nuScenes is defined as the BEV center distance between the prediction and the groud-truth. The overall AP is average AP in [0.5m, 1m, 2m and 4m].

\subsection{Implementation Details} \label{subsec:Implementation Details}
For all experiments except voxelization, we use the network architecture shown in \figref{fig:pointnet_backbone}. We shrink the number of embedding channels to $[64, 64, 512]$ in PointNet to achieve fast inference speed while maintaining accuracy. 512 points are sampled for each proposal. If the points number in one bounding box is fewer than 512, we randomly repeat the points to keep the input dimension. 
%We have tried to increase the input to 1024, but there is no additional performance benefit. 

For the voxelization experiments, we use two fully connected layer to extract features in each voxel. Then the features are max-pooled in voxels to form a $14\times 14 \times 14$ 3D voxel map. Finally, five 3D convolution layers and three fully-connected layers are utilized to extract the R-CNN features. 

To ensure the reproducibility of our algorithm, we use the code base of mmdetection3d\footnote{https://github.com/open-mmlab/mmdetection3d}
%and OpenPCDet~\footnote{https://github.com/open-mmlab/OpenPCDet} 
to extract proposals from Waymo Open Dataset. We directly save the outputs from PointPillars~\cite{pointpillars} and SECOND~\cite{second} with default testing settings in mmdetection3d as our inputs. There are about 7 million vehicle proposals, xx pedestrian proposals and yy cyclist proposals for each model. 

Besides the models from mmdetection3d, we also apply our proposed algorithm on the recently proposed RCD model~\cite{rcd}. It is a two-stage detector with a range view based first stage and a voxel-based second stage. Since it is not open-sourced, we only re-implemented its baseline model without the Range Conditioned Convolution operator. The results of both stages match with the original paper.

In our experiments, all models are trained using SGD with momentum of 0.9 for 60 epochs. The training schedule is a poly learning rate update strategy, starting from 0.02 with $10^{-5}$ weight decay. Training the model on WOD takes 7 hours on 4 Nvidia Geforce GTX2080Ti GPU with 256 batch size per GPU. 
%in which score threshold is 0.1, NMS threshold is 0.25

% As for nuScenes datasets, because there are 11 classes in this dataset, we get the outputs without nms with 0.1 score threshold to keep enough training samples.

\subsection{3D Detection on the Waymo Open Dataset} \label{subsec:Waymo Open Dataset}
On Waymo Open Dataset, we apply the proposed \Name to 3 different kinds of baseline models: Pointpillars~\cite{pointpillars}, SECOND~\cite{second}, and RCD~\cite{rcd} which are birds-eye-view based, 3D voxel based, and range view based, respectively. All these methods are evaluated with 3D mAP in two difficulty levels defined in the official evaluation, where the LEVEL\_1 objects should contain at least 5 points in each groud-truth bounding box while the LEVEL\_2 objects only need one single point.

~\tabref{tab:waymo-vehicle} reports the results of vehicle detection with 3D and BEV AP on validation sequences. Note that after hyperparameters finetuning, the performance of PointPillars~\cite{pointpillars} implemented by mmdetection3d already surpasses the previous state-of-the-art model PV-RCNN~\cite{pv-rcnn}. As shown in ~\tabref{tab:waymo-vehicle}, our method improves all the baseline models with a significant margin. Benchmark on various distance ranges shows that \Name generally improves the baseline consistently on all distances. Furthermore, with the strong Pointpillars baseline, \Name outperforms the PV-RCNN by $5.31\%$ mAP on the 3D vehicle detection task. For the range view model

Additionally, we show multi-class detection results with VEHICLE, PEDESTRIAN, and CYCLIST in ~\tabref{tab:waymo-3d}. Because we only obtain the multi-class results of Pointpillars and SECOND from publicly available codes, we test our method with these two baselines only. We use a multi-class classification loss and a class-agnostic regression loss for the three classes detection, without any other tuning. ~\tabref{tab:waymo-3d} demonstrates that our model also performs well in detecting small objects besides vehicles.


% \subsection{3D Detection on the nuScenes Dataset} \label{subsec:nuScenes}

\subsection{Ablation Studies} \label{subsec:Ablation}
In this section, we first conduct an ablation study to support the arguments on \secref{subsec:Problem}. And then, we show the generalization and inference time of proposed method. We show both single-class and multi-class results in Waymo Open Dataset in this section.

% \tabref{tab:ablation-vp} shows that different methods proposed in \secref{subsec:Problem} reach the similar results. All, however, sought the same end: to make the network scale-awarded. Not limited to these methods, other scale-awarded methods should also be effective. As our discussion in \secref{subsec:Problem}, the voxel and anchor based methods do not achieve good results while the normalization methods meet the performance
\textbf{Solution to the ambiguity problem}.
\tabref{tab:ablation-single} shows the comparison with different methods proposed in \secref{subsec:Problem}. From the table, we can conclude that all the point-based R-CNN models outperforms the baseline PointPillars. The PointNet models performs even better than voxel based models, which indicates that multi-layer convolution networks may lose the accurate point-level localization information. All other solutions achieve similar improvements compared with baseline on the one-class setting.

Nevertheless, when it comes to the multi-class problem, the size normalization and anchor solution suffer from difficulty in distinguishing different categories, which drops their performance (\tabref{tab:ablation-three}). The virtual point and offset methods, which fuly solve the ambiguity problem, reach the best results. 

In \tabref{tab:ablation-voxel}, we show the performance improvement of our \Name based on RCD model~\cite{rcd}. The RCD model is built with a voxel-based second stage, whose features are not only from the raw points, but also from the high level CNN feature maps. Similar with the voxel experiments in \tabref{tab:ablation-single}, the voxelization method is inferior to our purely point-based R-CNN model. 

%RCD model is built with a voxel-based second stagewe argue that coordinates include the most accurate information for location task. Following ~\cite{rcd}, we reproduced a range view based detector with a voxel-based second stage whose inputs include points' features extracted by the first stage. As shown, even using high-level features, the voxel-based method is still not as good as ours. The voxelization and 3D downsampling make the location ambiguous. 

%As discussed in \secref{subsec:Problem}, the PointNet baseline and voxel based methods do not achieve good results, while the normalization and anchor methods meet the performance of our proposed two methods due to the scale of most vehicles are similar.  Both, however, sought the same end: to make the network scale-awarded. Not limited to these methods, other scale-awarded methods should also be effective. 

\textbf{Network volumn}.
A trade-off between speed and accuracy can be achieved by modifing the channels in points encoding. To quantify the effect of channels, we show a \Name(2x) in \tabref{tab:waymo-3d} which obtains further $0.6\%$ improvement in pedestrian and $1.8\%$ in cyclist with two times channels. In addition, we also show the adaptive inference time by changing the number of sampled points per objects in \figref{fig:number_points}.


\textbf{Cross-model generalization}
\tabref{tab:ablation-generalization} demonstrates that our approach is able to generalize across models. Without finetuning, \Name trained on Pointpillars works well on SECOND model. 

\textbf{Target ablation}
\begin{table}
	\small 
	\begin{center}
		\scalebox{1}[1]{
			\setlength\tabcolsep{2pt}
			\begin{tabular}{l|cccc|cc}
				\hline
				Method & 
				\tabincell{c}{score} & 
				\tabincell{c}{center} &
				\tabincell{c}{size} &
				\tabincell{c}{heading} 
				& AP@L1 & AP@L2 \\
				\hline
				PointPillars~\cite{pointpillars} &  & & & &  72.1 & 63.6  \\ \midrule
				PointNet~\cite{pointnet} & \checkmark & & &   & 72.9 & 64.2   \\
				refinement&  & \checkmark & &  & 72.9 & 64.3  \\
				&  &  & \checkmark&  &  72.2 & 63.7  \\
				&  &  & & \checkmark &  72.1 & 63.6  \\ 
				%  \cline{2-7}
				&\checkmark  & \checkmark & \checkmark& \checkmark &  74.1 & 65.3  \\ \midrule
				\Name & \checkmark & & &   & 74.5 & 65.9   \\
				boudary offset&  & \checkmark & &  &  74.7 & 65.9  \\
				&  &  & \checkmark&  &  73.8 & 65.1  \\
				&  &  & & \checkmark &  73.4 & 64.6  \\
				%  \cline{2-7}
				&\checkmark  & \checkmark & \checkmark& \checkmark &  75.6 & 66.5  \\ 
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{Sub-task ablation study.}
	\label{tab:ablation-real}
\end{table}
A R-CNN model needs to do two tasks, namely classification task and regression task. The regression task can be further splitted into three sub-tasks, center regression, size regression and orientation regression. In \tabref{tab:ablation-real}, we successively add these tasks to see the effect of each sub-task. From the table, we can conclude that the vanilla PointNet refinement cannot improve the size and heading of the baseline PointPillars\cite{pointpillars} model. 


Finally, we show our inference time and model size in \tabref{tab:ablation-speed}. Memory and computational demands of \Name is marginal.



